Representation Learning on Variable Length and Incomplete Wearable-Sensory Time Series

The prevalence of wearable sensors (e.g., smart wristband) is creating unprecedented opportunities to not only inform health and wellness states of individuals, but also assess and infer personal attributes, including demographic and personality attributes. However, the data captured from wearables, such as heart rate or number of steps, present two key challenges: 1) the time series is often of variable-length and incomplete due to different data collection periods (e.g., wearing behavior varies by person); and 2) inter-individual variability to external factors like stress and environment. This paper addresses these challenges and brings us closer to the potential of personalized insights about an individual, taking the leap from quantified self to qualified self. Specifically, HeartSpace proposed in this paper encodes time series data with variable-length and missing values via the integration of a time series encoding module and a pattern aggregation network. Additionally, HeartSpace implements a Siamese-triplet network to optimize representations by jointly capturing intra- and inter-series correlations during the embedding learning process. The empirical evaluation over two different real-world data presents significant performance gains overstate-of-the-art baselines in a variety of applications, including personality prediction, demographics inference, and user identification.

==> fig/parameter_sensitivity_embedding.tex <==


























\begin{tikzpicture}
\begin{axis}[
    xlabel={Embedding Dimension $d_e$},
    ylabel={F1-score},
    xmin=32,xmax=256,
    ymin=0.7,ymax=1.0,
    xtick={32,64,128,256},
    xticklabels={32,64,128,256},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
    table[x=para, y=f1] {embedding_dimension_f1.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Embedding Dimension $d_e$},
    ylabel={Accuracy},
    xmin=32,xmax=256,
    ymin=0.7,ymax=1.0,
    xtick={32,64,128,256},
    xticklabels={32,64,128,256},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color=green!50!red, mark=diamond, dashed, mark options={solid}]
    table[x=para, y=acc] {embedding_dimension_acc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Embedding Dimension $d_e$},
    ylabel={AUC},
    xmin=32,xmax=256,
    ymin=0.8,ymax=1.0,
    xtick={32,64,128,256},
    xticklabels={32,64,128,256},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,1;green,2;blue,3}, mark=x, dashed, mark options={solid}]
    table[x=para, y=auc] {embedding_dimension_auc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


==> fig/parameter_sensitivity_negative_set.tex <==


























\begin{tikzpicture}
\begin{axis}[
    xlabel={Negative Query Size $S_p$},
    ylabel={F1-score},
    xmin=2,xmax=10,
    ymin=0.7,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
    table[x=para, y=f1] {num_negative_f1.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Negative Query Size $S_p$},
    ylabel={Accuracy},
    xmin=2,xmax=10,
    ymin=0.7,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color=green!50!red, mark=diamond, dashed, mark options={solid}]
    table[x=para, y=acc] {num_negative_acc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Negative Query Size $S_p$},
    ylabel={AUC},
    xmin=2,xmax=10,
    ymin=0.8,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,1;green,2;blue,3}, mark=x, dashed, mark options={solid}]
    table[x=para, y=auc] {num_negative_auc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


==> fig/parameter_sensitivity_positive_set.tex <==


























\begin{tikzpicture}
\begin{axis}[
    xlabel={Positive Query Size $S_p$},
    ylabel={F1-score},
    xmin=2,xmax=10,
    ymin=0.7,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
    table[x=para, y=f1] {num_positive_f1.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Positive Query Size $S_p$},
    ylabel={Accuracy},
    xmin=2,xmax=10,
    ymin=0.7,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color=green!50!red, mark=diamond, dashed, mark options={solid}]
    table[x=para, y=acc] {num_positive_acc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Positive Query Size $S_p$},
    ylabel={AUC},
    xmin=2,xmax=10,
    ymin=0.8,ymax=1.0,
    xtick={2,4,6,8,10},
    xticklabels={2,4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,1;green,2;blue,3}, mark=x, dashed, mark options={solid}]
    table[x=para, y=auc] {num_positive_auc.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}


==> fig/parameter_sensitivity_reference_set.tex <==


























\begin{tikzpicture}
\begin{axis}[
    xlabel={Reference Set Size $S_r$},
    ylabel={F1-score},
    xmin=4,xmax=10,
    ymin=0.7,ymax=1.0,
    xtick={4,6,8,10},
    xticklabels={4,6,8,10},
    % legend columns=2,
    legend cell align=right,
    grid=both,
    %ylabel style={align=center},
    ylabel style={align=center},
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=2.15},
    label style={scale=2.3},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(0,0)},anchor=south west},
    every axis plot post/.append style={
        every mark/.append style={scale=3.5}
    }
]

\addplot[color={rgb:red,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
    table[x=para, y=f1] {num_reference_f1.txt};
%\legend{\Large F1, \Large ACC, \Large AUC};

\end{axis}
\end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     xlabel={Reference Set Size $S_r$},
%     ylabel={Accuracy},
%     xmin=4,xmax=10,
%     ymin=0.7,ymax=1.0,
%     xtick={4,6,8,10},
%     xticklabels={4,6,8,10},
%     % legend columns=2,
%     legend cell align=right,
%     grid=both,
%     ylabel style={align=center},
%     every axis plot/.append style={ultra thick},
%     every tick label/.append style={scale=2.15},
%     label style={scale=2.3},
%     legend style={
%         nodes={scale=1.5, transform shape},
%         legend image post style={scale=1.5},
%         },
%     legend style={at={(0,0)},anchor=south west},
%     every axis plot post/.append style={
%         every mark/.append style={scale=3.5}
%     }
% ]

% \addplot[color=green!50!red, mark=diamond, dashed, mark options={solid}]
%     table[x=para, y=acc] {num_reference_acc.txt};
% %\legend{\Large F1, \Large ACC, \Large AUC};

% \end{axis}
% \end{tikzpicture}


% \begin{tikzpicture}
% \begin{axis}[
%     xlabel={Reference Set Size $S_r$},
%     ylabel={AUC},
%     xmin=4,xmax=10,
%     ymin=0.7,ymax=1.0,
%     xtick={4,6,8,10},
%     xticklabels={4,6,8,10},
%     % legend columns=2,
%     legend cell align=right,
%     grid=both,
%     ylabel style={align=center},
%     every axis plot/.append style={ultra thick},
%     every tick label/.append style={scale=2.15},
%     label style={scale=2.3},
%     legend style={
%         nodes={scale=1.5, transform shape},
%         legend image post style={scale=1.5},
%         },
%     legend style={at={(0,0)},anchor=south west},
%     every axis plot post/.append style={
%         every mark/.append style={scale=3.5}
%     }
% ]

% \addplot[color={rgb:red,1;green,2;blue,3}, mark=x, dashed, mark options={solid}]
%     table[x=para, y=auc] {num_reference_auc.txt};
% %\legend{\Large F1, \Large ACC, \Large AUC};

% \end{axis}
% \end{tikzpicture}



==> solution.tex <==


\section{Methodology: \emph{\model}}
\label{sec:solution}

% Generally speaking, our \model\ model consists of three key components: i) day-specific time series encoder; ii) pattern aggregation networks; iii) 
% To handle the representation learning with variable-length input, we propose a segmentation and aggregation approach on time series data. 

\begin{figure}
    \centering
    \vspace{-0.15in}
    \includegraphics[width=0.7\textwidth]{fig/framework.pdf}
    \vspace{-0.25in}
    \caption{\model\ Framework. The training flow can be summarized as: (1) partition raw sensory data to a set of day-long time series; (2) map each day-long time series into a representation vector by Day-Specific Time Series Encoding Module (3) fuse day specific representations through Temporal Pattern Aggregation Network (4) update parameters based on reconstruction loss and Siamese-triple loss.}
    \label{fig:autoencoder}
    \vspace{-0.1in}
\end{figure}

\emph{\model} consists of three key components: i) Day-specific time series encoding; ii) Temporal pattern aggregation network; and iii) Siamese-triplet network optimization strategy.

%We first introduce the key ingredients of our \model\ framework in details and then discuss the model inference.

%\vspace{-0.1in}
%\paragraph{Time Series Segmentation}
Considering that periodicity has been demonstrated as an important factor that governs human sensory data (\eg, heart rate) with time-dependent transition regularities~\cite{nakamura2018cross}, and the sensed time series data are often variable-length, we first partition the wearable-sensory time series (\ie, $\textbf{X}_i$) of each user $u_i$ into $T$ (indexed by $t$) separated day-long time series ($T$ may vary among users). %The definition of each individual day-long time series is given as follows:

\begin{Dfn}
\textbf{Day-long Time Series $\textbf{x}_i^t$}. Each $t$-th divided day-long time series of $\textbf{X}_i$ is denoted as $\textbf{x}_i^t \in \mathbb{R}^{K}$, where $K$ is the number of time steps included in one day. In $\textbf{x}_i^t$, each element $\textbf{x}_i^{t,k}$ represents the sensed measurement from user $u_i$ at the $k$-th time step in $\textbf{x}_i^t$. Due to the data incompleteness issue of the collected time series, we set the element $\textbf{x}_i^{t,k}$ as zero to keep equally-spaced intervals if there is no measurement collected from user $u_i$ at the $k$-th time step in $\textbf{x}_i^t$.
\end{Dfn}

\vspace{-0.1in}
\subsection{Day-Specific Time Series Encoding}
To explore the underlying repeated local patterns and reduce dimensions of day-long time series data, we first propose a convolution autoencoder module to map each individual series $\textbf{x}_i^t$ into a common low-dimensional latent space. In general, the encoder first takes day-long time series as the input and then translates it into a latent representation which encodes the temporal pattern. Then, the decoder network reconstructs the data which is identical with the input $\textbf{x}_i^t$ in the ideal case. 
% To encode complex sequential transition regularities of the high-dimensional day-long time series data with missing values, we first propose a deep autoencoder module to map each individual series $\textbf{x}_i^t$ into a common low-dimensional latent space. In general, the encoder first takes day-long time series as the input and then translates it into a latent representation which encodes the temporal pattern. Then, the decoder network reconstructs the data which is identical with the input $\textbf{x}_i^t$. 
To keep the input dimension consistent with complete day-specific time series, we apply zero padding by filling in zero value to missing observations. However, it may bring in the negative effect in the encoding process. Since the filled value are treated equally as other valid inputs when apply kernels in each convolutional layer, the generated features may incorrectly encoded and further lead to the error propagation from low to high layers. To mitigate the undesired effects from zero padding, we propose a dual-stage gating mechanism by re-weighting hidden units in each layer.
% To alleviate the data incompleteness issue, we develop a dual-stage gating mechanism which is tailored to integrate with our deep autoencoder architecture. In order to jointly capture the channel-wise and temporal dependencies across time steps and channel dimensions.
More specifically, each layer of our deep autoencoder framework is a four-step block: i) convolution network; ii) channel-wise gating mechanism; iii) temporal gating mechanism; and iv) pooling operation. Figure~\ref{fig:autoencoder} presents the architecture of our deep autonencoder module.

\subsubsection{\bf Convolutional Neural Network}
Firstly, we apply convolutional neural network (CNN) to encode the local pattern of day-long time series $\textbf{x}_i^t$. Specifically, we feed $\textbf{x}_i^t$ into a number of convolutional layers. Let's denote $\mathcal{V}_{i,t}^{l-1} \in \mathbb{R}^{d_k^{l-1} \times d_c^{l-1}}$ as the feature map representation of $(l-1)$-th layer, where $d_c^{l-1}$, $d_k^{l-1}$ indicates the channel dimension, temporal dimension size in $(l-1)$-th layer, respectively. $i$ and $t$ is user and day index, respectively. Formally, the output of $l$-th layer in our CNN is given as:
\begin{align}
\mathcal{V}_{i,t}^l = f(\textbf{W}^l_c * \mathcal{V}_{i,t}^{l-1} + \textbf{b}^l_c)
\end{align}
\noindent where $f(\cdot)$ is the activation function and $*$ denotes the convolutional operation. $\textbf{W}^l_c$ and $\textbf{b}^l_c$ represents the transformation matrix and bias term in $l$-th layer of the CNN, respectively. 

%model low dimensional latent characteristics of each day-long time series.
% In \model, we first propose an Time Series Representations component to express temporal patterns of each day-long time series, which adopts the autoencoder architecture. In general, the autoencoder is an unsupervised learning structure to learn low dimensional representations from input data. 
% Then, the decoder uncompress the representation that closely match \red{matches} the original input. We found it important to connect each layer with dual-stage gating mechanisms which alleviate the influence caused by data incomplete \red{incompleteness} to each unit in the next layer. Figure \red{missing reference here} \label{fig:autoencoder} shows the architecture of our proposed autoencoder.

% To address the data incompleteness challenge, we design a deep framework to encode the inputs into continuous latent representations with the preservation of complex temporal structure property.

% There exist two key challenges in order to learn effective embeddings: (i) This automatically encoding process is non-trivial since the missing data period of different users can be quite different (the missing measuÆ’rements will be set as 0 in $\boldsymbol{X}_{i}^t$). It is not reasonable to treat elements of different time steps equally during the encoding process. Hence, we need to carefully decide the importance weight of each time step to generate latent low-dimensional representations. (ii) Furthermore, there exist implicit dependencies across different channels of intermediate representations and channel-specific patterns interweave with each other in a hierarchical way. Capturing such inter-dependencies remains a significant challenge.

% To address the above challenges, we propose to integrate a dual-stage recalibration gating mechanism with a convolutional network network to encode the input time series $\boldsymbol{X}_{i}^t$ into continuous latent representations. In particular, each block of our deep autoencoder framework is a four-step module: i) convolution encoder; ii) channel-wise gating mechanism; iii) temporal gating mechanism; iv) pooling operation. Figure~\ref{fig:autoencoder} represents the architecture of our deep autoencoder model.

\subsubsection{\bf Channel-Wise Gating Mechanism} 
In our deep autoencoder module, the goal of the channel-wise gating mechanism is to re-weight hidden units by exploiting the cross-channel dependencies and select the most informative elements from the encoded feature representation $\mathcal{V}_{i,t}$~\cite{hu2018squeeze}.To exploit the dependencies over channel dimension, we first apply temporal average pooling operation $\textbf{F}_{pool}^{cg}(\cdot)$ on the feature representation $\mathcal{V}_{i,t}$ over temporal dimension ($1\!\!\leq\!\! k\!\!\leq\!\! K$) to produce the summary of each channel-wise representation as:
\begin{align}
\textbf{z}_{i,t}^{cg} = \textbf{F}_{pool}^{cg}(\mathcal{V}_{i,t}) = \frac{1}{K} \sum_{k=1}^K \mathcal{V}_{[k,:]};~\textbf{z}_{i,t}^{cg} \in \mathbb{R}^{d_c}
\label{equ:channel_1}
\end{align}
\noindent where $\textbf{z}_{i,t}^{cg}$ represents the intermediate representation of $\mathcal{V}_{i,t}$ after average pooling operation over temporal dimension. Then, our channel-wise gating mechanism recalibrates the information distribution among all elements across channels as:
\begin{align}
\textbf{a}_{i,t}^{cg} = \text{Sigmoid} (\textbf{W}_2^{cg} \cdot \text{ReLU}(\textbf{W}_1^{cg} \cdot \textbf{z}_{i,t}^{cg}));~\textbf{a}_{i,t}^{cg} \in \mathbb{R}^{d_c}
\label{equ:channel_2}
\end{align}
\noindent where $\textbf{a}_{i,t}^{cg}$ denotes the channel-wise importance vector in which each entry is the each channel's importance. $\textbf{W}_1^{cg}$ and $\textbf{W}_2^{cg}$ is the learned transformation matrix of two fully connected neural-net layers. Finally, the channel-wise representations $\widetilde{\mathcal{V}}_{i,t}$ is learned as:
\begin{align}
\widetilde{\mathcal{V}}_{i,t} = \textbf{F}_{scale}(\mathcal{V}_{i,t},\textbf{a}_{i,t}^{cg}) = \mathcal{V}_{i,t} \odot \textbf{a}_{i,t}^{cg}
\label{equ:channel_3}
\end{align}
\noindent where $\odot$ is the element-wise production operation.
%where $\mathcal{V}_{i,j} \in \mathbb{R}^{K\times d_c}$ and $\mathcal{V}_{i,j}^a$ is the $a$-th vector of the original representation $\mathcal{V}_{i,j}$.



% \subsubsection{\bf Temporal-wise Gating Mechanism}
% To re-weight the hidden units by capturing the temporal dependencies of feature representation across time steps, we also apply a gating mechanism on temporal dimension to further learn focus points in the time-ordered internal feature representation $\widetilde{\mathcal{V}}_{i,t}$ (output from the channel-wise gating mechanism).
% % Formally, the channel average pooling operation $\textbf{F}_{pool}^{tg}(\cdot)$ on the feature representation $\widetilde{\mathcal{V}}_{i,t}$ over channel dimension (indexed by $c$, $1\leq c\leq d_c$) is applied to generate one-dimensional vector.
% Formally, our temporal-wise gating mechanism can be represented as follows:
% % Particularly, our temporal gating mechanism aims to capture the relevance of $\widetilde{\mathcal{V}}_{i,j}$ across different time steps.
% % \begin{align}
% % \textbf{z}_{i,t}^{tg} = \textbf{F}_{pool}^{tg}(\widetilde{\mathcal{V}}_{i,t}) = \frac{1}{d_c} \sum_{c=1}^{d_c} \widetilde{\mathcal{V}}_{[:,c]};~\textbf{z}_{i,t}^{tg} \in \mathbb{R}^{K}
% % \end{align}
% % \noindent $\textbf{z}_{i,t}^{tg}$ is the intermediate representation after average pooling operation over channel dimension. Formally, our temporal-wise gating mechanism can be represented as follows:
% \begin{align}
% \textbf{z}_{i,t}^{tg} &= \textbf{F}_{pool}^{tg}(\widetilde{\mathcal{V}}_{i,t}) = \frac{1}{d_c} \sum_{c=1}^{d_c} \widetilde{\mathcal{V}}_{[:,c]}\\
% \textbf{a}_{i,t}^{tg} &= \text{Sigmoid} (\textbf{W}_2^{tg} \cdot \text{ReLU}(\textbf{W}_1^{tg} \cdot \textbf{z}_{i,t}^{tg}))\\
% \widetilde{\mathcal{V}}_{i,t}^* &= \textbf{F}_{scale}(\widetilde{\mathcal{V}}_{i,t},\textbf{a}_{i,t}^{tg}) = \widetilde{\mathcal{V}}_{i,t}\odot \textbf{a}_{i,t}^{tg}
% \end{align}
% \noindent where $\textbf{a}_{i,t}^{tg}$ represents the temporal relevance vector. $\textbf{W}_1^{tg}$ and $\textbf{W}_2^{tg}$ is the learned transformation matrices. We output the $\widetilde{\mathcal{V}}_{i,t}^* \in \mathbb{R}^{d_c}$ as the summarized feature representation which jointly preserve the channel-wise and temporal dependencies.


\subsubsection{\bf Temporal-wise Gating Mechanism}
To re-weight the hidden units by capturing the temporal dependencies of feature representation across time steps, we also apply a gating mechanism on temporal dimension to further learn focus points in the time-ordered internal feature representation $\widetilde{\mathcal{V}}_{i,t}$ (output from the channel-wise gating mechanism).
Similar to the gating mechanism procedures encoded in Equations~\ref{equ:channel_1}, \ref{equ:channel_2}, and \ref{equ:channel_3},
we first apply the channel average pooling operation on feature representation $\widetilde{\mathcal{V}}_{i,t}$ over channel dimension and get $\widetilde{\mathcal{V}}_{i,t}^* \in \mathbb{R}^{d_c}$ as the summarized feature representation which jointly preserve the channel-wise and temporal dependencies.

%\ie, $s_t^b\in S_t (1\leq b \leq K)$

%Add itemlizes

\subsubsection{\bf Encoder-Decoder Configuration} We present the architecture configuration of our deep autoencoder module.\\\vspace{-0.1in}

\noindent \textbf{Encoder}. Given the day-long time series $\textbf{x}_i^t \in \mathbb{R}^K$ (we set $K=1440$), we use ReLU activation function and contain $5$ convolutional layers (\ie, Conv1-Conv5) followed by channel-wise, temporal-wise gating mechanism and pooling layers. Particularly, Conv1-Conv5 is configured with the one-dimensional kernel with $\{9,7,7,5,5\}$ and filter sizes with $\{32,64,64,128,128\}$, respectively. Then, we perform the flatten operation on the output to generate a one-dimensional feature representation and feed it into a fully connected layer with $Tanh$ activation function to generate the final latent representation $\Psi_{i}^t$ corresponding to the time series $\textbf{x}_{i}^t$. \\\vspace{-0.1in}

\noindent \textbf{Decoder}. The decoder is symmetric to the encoder in terms of layer structure. First, the representation $\Psi_i^t$ is uncompressed by a single-layer with $Tanh$ activation function and then followed by a series of five deconvolutional layers with ReLU activation function. The kernel and filter sizes is in reverse order to be symmetric to the encoder architecture configuration. Channel-wise and Temporal-wise are applied in the first four layer after deconvolutional operation.\\\vspace{-0.1in}

% Our deconvolutional module is consisted of a number of transposed convolutional layers to generate the latent feature representations in our autoencoder framework. Specifically, we perform max pooling operation on the encoded feature representation $\widetilde{\mathcal{V}}_{i,j}^*$. We finally conduct flattern operation on the representation matrix $\widetilde{\mathcal{V}}_{i,j}^*$ to transform it into a one-dimensional vector and further fed it into a Multilayer Perceptron~\cite{he2017neural} to generate the final latent representation $\Psi_{i,j}$ of day-long time series $\boldsymbol{X}_{i}^t$. In the decoder, we apply the aforementioned four key steps in reverse order to be symmetric with the encoder framework, \ie, deconvolutional module $\rightarrow$ temporal gating mechanism $\rightarrow$ channel-wise gating mechanism $\rightarrow$ convolutional encoder. Formally, the loss function of our autoencoder framework is formally defined as follows:

\noindent \textbf{Loss Function in Deep Autoencoder Module}: We formally define the reconstruction loss function in our deep autoencoder module as follows:
%We train our deep autoencoder by regressing to the measurement. The loss function is formally defined as follows:
\begin{align}
\mathcal{L}_{ae} = ||M \odot (D(E(\textbf{x}_i^t)) - \textbf{x}_i^t)||^2_2
\end{align}
\noindent where $M \in \mathbb{K}$ is a binary mask vector corresponding to each element in $\textbf{x}_i^t$. In particular, 
$M_k=1$ if $x_i^{t,k}\neq 0$(i.e., has measurement) and $M_k=0$ otherwise. $\odot$ is the element-wise product operation, $\textbf{x}_{i}^t$ is the input, $E(\cdot)$ and $D(\cdot)$ represents the encoder and decoder function.

%collected value with 1 and 0 for missing value in each timestamp, 

\begin{figure}
    \centering
    \vspace{-0.15in}
    \includegraphics[width=0.8\textwidth]{fig/auto-encoder.pdf}
    \vspace{-0.10in}
    \caption{Illustration of Day-Specific Time Series Encoding.}
    \label{fig:autoencoder}
    \vspace{-0.2in}
\end{figure}

\vspace{-0.1in}
\subsection{Temporal Pattern Aggregation Network}
While applying the autoencoder framework to map day-long time series $\textbf{x}_i^t$ of variable-length into a low-dimensional latent representation $\Psi_{i}^t$, how to appropriately fuse day-specific temporal patterns still remains a significant challenge. To address this challenge and aggregate the encoded temporal-wise patterns, we develop a temporal pattern aggregation network which promotes the collaboration of different day-specific temporal units for conclusive cross-time representations. Figure~\ref{fig:fusion_process} shows the architecture of our temporal pattern aggregation network which consists of three major modules: i) Context-aware time embedding module; ii) multi-head aggregation network; iii) temporal attention network.

% The key idea of aggregator component is to fuse daily features compressed from TS auto-encoder for variable-length time series data. In particular, we integrate embedding vectors learned from each daily-long chunks into a new embedding vectors by jointly considering the relatively time difference and behavior similarity across different time chunks.      

% To learn a conclusive representation

%\vspace{-0.1in}
\subsubsection{\bf Context-Aware Time Embedding Module}
% refer to Deep Semantic Role Labeling with Self-Attention
% https://arxiv.org/pdf/1706.03762.pdf(refer section 3)
% application: Deep Semantic Role Labeling with Self-Attention
% To incorporate temporal contextual signals into our learning framework, we further augment our model with a time-aware embedding module to differentiate individual dates. In real-world scenarios, different people may exhibit different health-sensory data distribution due to their various daily routines~\cite{probst2016emotional}. For example, an office worker may exhibit a strong periodicity on the heart rate records due to his/her regular periodic activities, while the heart rate distribution of a freelancer may have different personalized transition regularities over different periods, because of his/her irregular daily routines and activities~\cite{stirn2006prevalence}. To address this problem in our time-aware embedding module, we consider the relative time difference between the last time step and other previous time steps in our model. For example, given a health-sensory time series with a date vector of three measured timestamp information $[2018/10/01, 2018/10/20, 2018/10/25]$, we generate a new date duration vector using the date duration information as $[24, 5, 0]$ (the day duration between 2018/10/01 and 2018/10/25 is 24 days). Based on the generated date duration vector, in order to avoid the inconsistency between training and testing instances with respect to long date duration, we propose to assign the each element of the date duration vector with a fix (non-trainable) date embedding using the timing signal approach~\cite{vaswani2017attention}. Formally, the embedding vector $E_j$ of $j$-th day is estimated as follows:
From the deep autoencoder module, given the time series $\textbf{X}_i$ of user $u_i$, we learn a set of date-ordered latent representations with size of $T$, \ie, $\Psi_{i} = <\Psi_{i,1},...,\Psi_{i,t},...,\Psi_{i,T}>$.
In the real world, different people may exhibit different wearable-sensory data distribution due to specific daily routines~\cite{probst2016emotional}. To incorporate the temporal contextual signals into our learning framework, we further augment our model with a time-aware embedding module, which utilizes the relative time difference between the last time step and each previous one. For example, given a time series with three date information $\{$2018-10-01, 2018-10-20, 2018-10-25$\}$, we generate a date duration vector as $\{24, 5, 0\}$ (the day duration between 2018-10-01 and 2018-10-25 is $24$ days). To avoid inconsistency between training and test instances with respect to long date duration, we assign to each element of the vector a fix (non-trainable) date embedding using the timing signal method~\cite{vaswani2017attention}. The embedding vector $\textbf{e}_t$ of $t$-th day is derived as:
\begin{align}
e_{t, 2i} = \text{sin}(\frac{t}{10000^{2i/d_e}});~~e_{t, 2i+1} = \text{cos}(\frac{t}{10000^{2i/d_e}})
\end{align}
\noindent where $t$ is the relative time value and $d_e$ is the embedding dimension ($2i+1$ and $2i$ are the odd and even index in the embedding vector). New context-aware latent vector $\textbf{h}_{i,t} \in \mathbb{R}^{d_e}$ is generated by element-wise adding each day-specific feature representation $\Psi_{i}^t$ and date embedding $\textbf{e}_t$, to incorporate the temporal contextual signals into the learned embeddings.
%which is indexed by $e$. $j$ represents date index.

% Jointly considering people's behavior (heart rate) and time series may also reveals user's information\cite{}. For example, an office worker may exhibits a strong weekly repeated pattern on his heart rate time series data with strong work intensity during weekdays and relaxed time on weekends. In contrast, a freelancer may have a relatively irregular life. So, the aggregation requires the information about the relative time distance between chunked time series input. For example, the heart rate time series is collected from $[2018/10/01, 2018/10/20, 2018/10/25]$, the relative time position is $[24, 5, 0]$. There are many choices to encode the embedding vector. In order to extrapolate to relatively time difference longer than the ones encountered during training, we utilize the fix(non-trainable) date embedding by timing signal approach proposed in \cite{vaswani2017attention}:
% \begin{align}
% \textbf{TE}_{t, 2i} = sin(t/10000^{2i/dim}) \nonumber\\
% \textbf{TE}_{t, 2i+1} = cos(t/10000^{2i/dim})
% \end{align}
% \noindent where $t$ is the relative time position, $i$ is the index of embedding dimension, $dim$ is the dimension of time embedding.  

% To 
% The date of collected day-long time series chunk provides information and  The representation learning itself cannot distinguish between different dates. 

\subsubsection{\bf Multi-Head Aggregation Network}
% https://arxiv.org/pdf/1808.09781.pdf


During the pattern fusion process, we develop a multi-head attention mechanism which is integrated with a point-wise feedforward neural network layer, to automatically learn the quantitative relevance in different representation subspaces across all context-aware temporal patterns). %More specifically, given the time series $\textbf{X}_i$ of user $u_i$, we learn a set of date-ordered latent representations with size of $T$, \ie, $\Psi_{i} = <\Psi_{i,1},...,\Psi_{i,t},...,\Psi_{i,T}>$. We generate a new context-aware latent vector $\textbf{h}_{i,t} \in \mathbb{R}^{d_e}$ by element-wise adding each day-specific feature representation $\Psi_{i}^t$ and date embedding $E_t$, to incorporate the temporal contextual signals into the learned embeddings.
Specifically, given the $i$-th time series, we feed all context-aware day-specific embeddings $\textbf{H}_{i} = \{\textbf{h}_{i,0}, \cdots, \textbf{h}_{i,T}\}$ into a multi-head attention mechanism. Here, $M$-heads attention conducts the cross-time fusion process for $M$ subspaces ($m\in [1,...,M]$). Each $m$-th attention operation involves a separate self-attention learning among $\textbf{H}_{i}$ as follows:
\begin{align}
% \widetilde{\textbf{H}}_{i,j} = \text{Self-Att}(\textbf{H}_{i,j}) = \text{softmax}(\frac{\textbf{H}_i \cdot \textbf{W}_1^{m} (\textbf{H}_i \cdot \textbf{W}_2^{m})^T}{\sqrt{d_m}}) \textbf{H}_i \cdot \textbf{W}_3^{m},
\widetilde{\textbf{H}}_{i}^m = \text{softmax}(\frac{ \textbf{W}_1^{m} \cdot \textbf{H}_{i}(\textbf{W}_2^{m} \cdot \textbf{H}_{i})^T }{\sqrt{d_m}}) \textbf{W}_3^{m} \cdot \textbf{H}_{i} ,
\end{align}
where $\textbf{W}_1^{m}, \textbf{W}_2^{m}, \textbf{W}_3^{m} \in \mathbb{R}^{d_m \times d_e }$ represent the learned parameters of $m$-th head attention mechanism, and $d_m$ is the embedding dimension of $m$-th head attention,\ie, $d_m = d_e/M$. Then, we concatentate each learned embedding vector $\widetilde{\textbf{H}}_{i}^m$ from each $m$-th head attention, and further capture the cross-head correlations as follows:
\begin{align}
% \widetilde{\textbf{H}}_{i,j}^c = \text{MultiHead}(\widetilde{\textbf{H}}) = concat(\widetilde{\textbf{H}}_{i,j}^1,...,\widetilde{\textbf{H}}_{i,j}^m,...,\widetilde{\textbf{H}}_{i,j}^M) \cdot  \textbf{W}_{cross}
\widetilde{\textbf{H}}_{i}^c = \textbf{W}_{c} \cdot concat(\widetilde{\textbf{H}}_{i}^1,...,\widetilde{\textbf{H}}_{i}^m,...,\widetilde{\textbf{H}}_{i}^M)   
\end{align}
$W_{c}\in \mathbb{R}^{d_e\times d_e}$ is the transformation matrix to model the correlations among head-specific embeddings. Hence, we jointly embed multi-modal dependency units into the space with the fused $\widetilde{\textbf{H}}_{i}^c$ using the multi-head attention network. The advantage of our multi-head attention network lies in that it allows the exploration of feature modeling in different representation spaces~\cite{zhang2018gaan}. Then, we further feed the fused embedding $\widetilde{\textbf{H}}_{i}^c$ into a feed-forward neural network:
\begin{align}
\widetilde{\textbf{H}}_{i}^f =\textbf{W}_2^f \cdot \text{ReLU}(\textbf{W}_1^f \cdot \widetilde{\textbf{H}}_{i}^c +\textbf{b}_1^f)+\textbf{b}_2^f,
\end{align}
where $\textbf{W}_1^f$, $\textbf{W}_2^f$ and $\textbf{b}_1^f$, $\textbf{b}_2^f$ are the weight matrix and bias in the feed-forward layer. In our \model\ framework, we perform multi-head attention mechanism twice.

\subsubsection{\bf Temporal Attention Network}
To further summarize the temporal relevance, we develop a temporal attention network to learn importance weights across time. Formally, our temporal attention module can be represented as follows:
% \begin{align}
% \label{equ:query_attention_u}
%  \widetilde{\textbf{h}}_{i,t}^a = \text{Tanh}(\textbf{W}^{a} \cdot \widetilde{\textbf{h}}_{i,t}^f +\textbf{b}^{a}).
% \end{align}
\begin{align}
\label{equ:query_attention_weight}
% \alpha_{i,t} = \frac{\exp{( \textbf{c}\cdot (\widetilde{\textbf{h}}_{i,t}^a)^T)}}{\sum_{t'\in [1,...,T]} \exp{(\textbf{c}\cdot (\widetilde{\textbf{h}}_{i,t'}^a )^T )}};~~~\widetilde{\Psi}_{i} = \sum_{t} \alpha_{i,t} \cdot \Psi_{i}^t
\boldsymbol{\alpha}_i &= \text{softmax}(\textbf{c}\cdot \text{Tanh}(\textbf{W}^{a} \cdot \widetilde{\textbf{H}}_{i}^f +\textbf{b}^{a}));~\widetilde{\Psi}_{i} = \sum_{t} \alpha_{i,t} \cdot \Psi_{i}^t
\end{align}
% \begin{equation}
% \label{equ:session_vector}
% \widetilde{\Psi}_{i} = \sum_{t} \alpha_{i,t} \cdot \Psi_{i}^t.
% \end{equation}
\noindent Output $\widetilde{\textbf{H}}_i^f$ is first fed into a one-layer neural network and then together with the context vector $\textbf{c}$ to generate the importance weights $\boldsymbol{\alpha}_i$ through the softmax function. The aggregated embedding $\widetilde{\Psi}_{i}$ is calculated as a weighted sum of day-specific embeddings based on the learned importance weights. For simplicity, we denote our temporal pattern aggregation network as $\widetilde{\Psi}_{i}=\textbf{A}(\Psi_i^{1},\cdots,\Psi_i^T)$.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{fig/multhead-attention.pdf}
    \caption{Temporal Pattern Aggregation Network.}
    \label{fig:fusion_process}
\end{figure}

%\red{equation 13 represents the softmax operation, equation 9 directly use the term softmax. Shall we be consistent here?}



% Equations~\ref{equ:query_attention_u}, ~\ref{equ:query_attention_weight}, and~\ref{equ:session_vector} summarize the aggregated embedding calculation.


%learned latent representation $\Psi_{i,j}$ of $j$-th day-specific time series from user $u_i$, we first .

% To fuse multiple time series embedding with relative time difference information, we first adopt multi-head attention followed by pointwise feed forward layer. And then we feed the temporal-information to get the importance weight of each time-series. 
% The aggregated embedding is the weighted sum of time series embeddings.

% Given a sequence of $n$ heart rating embeddings, denoted as $H = <h_0$, ..., $h_i$, ..., $h_n>$, where $i$ indicates the relative time position in the sequence, we first construct the positional heart rating embeddings by concatenating the heart rating embedding $h_i$ with its corresponding time embedding.
% The heart rating embedding at position $i$ is represented by $\hat{h}_i$.
% $\hat{h} \in R^{n \times d_{model}}$

% These positional heart rating embeddings are then fed into a multi-head attention to learn the importance weights by investigating the relative relationships among them.

% k-heads attention conducts the attention operations for $k$ times.
% Each time the attention operation $head_i$ involves a separate relational learning among $\hat{h}$.
% \begin{align}
% head_i = SelfAttention(H) = softmax(\frac{H \textbf{W}_{i}^{Q}(HW_{i}^{K})^T}{\sqrt{d_k}}) H \textbf{W}_i^{V},
% \end{align}
% where $W_^Q, \textbf{W}_i^K, \textbf{W}_i^{V} \in R^{d_{model} \times d_k}$, and $d_k = d_{model}/K$. We compute the dot products of the query with all keys, divide each by $\sqrt{d_k}$, and apply a softmax function to obtain the weights on the values $V$.
% \begin{align}
% P = MultiHead(H) = concat(head_1, ..., head_k) W^{O},
% \end{align}
% where $W^O \in R^{kd_v \times d_{model}}$, and $k$ is the number of heads in the attention mechanism.
% Multi-head attention allows the model to jointly attend to information from different representation subspaces at different time.


% [The output of each sub-layer is LayerNorm(x+Sublayer(x)), where sublayer(x) is the function implemented by the sub-layer itself.]

% The output of the multi-head attention layer is further fed into a feed-forward neural network.
% \begin{align}
% T =\textbf{ReLU}(PW + b)W'+b',
% \end{align}
% where $W$ and $b$ are the weight matrix and bias in the feed-forward layer, and $\sigma$ is the activation function.

% We repeat the multi-head attention for twice.


% The output $T$ of the feed-forward layer is used to yield the importance weights for the time series data.



%The aggregated embedding a weighted sum of the time series data.
%\begin{align}
%Emb_{aggregated} = \sum_{i} \textbf{W}_i emb(h_i)
%\end{align}

\vspace{-0.1in}
\subsection{Siamese-triplet Network Optimization Strategy}
% refer this paper https://arxiv.org/pdf/1505.00687.pdf
%(Triplet network)

Our goal is to embed each individual wearable-sensory time series into low-dimensional spaces, in which every time series is represented as an embedding vector. We develop a Siamese-triplet network optimization strategy to jointly model the structural information of intra-series temporal consistency and inter-series correlations in our learning process. In particular, within a series of sensing data points (\eg, heart rate records), even though the measurements change over time, they do not change drastically within a short time period, since they belong to the same user~\cite{ukil2016heart}. Additionally, the heart rate measurements sampled from consecutive time intervals (\eg, days) of the same people may a more similar distribution as compared to sampling from different people~\cite{bhattacharjee2018heart}. Motivated by these observations, the key idea of our Siamese-triplet network optimization framework is to learn representations with the constrain--making intra-series data point pairs closer to each other and inter-series data point pairs further apart. We first define the following terms to be used in our optimization strategy.\vspace{-0.05in}
\begin{Dfn}
\textbf{Reference Set $\textbf{R}_i$}: we define $\textbf{R}_i$ to represent the sampled reference set of user $u_i$. In particular, $\textbf{R}_i = \{\textbf{r}_i^1,\cdots,\textbf{r}_i^{S_r}\}$ , where $S_r$ is size of reference set corresponding to $S_r$ sampled day-specific time series from $\textbf{X}_i$. Each entry in $\textbf{R}_i$ represents the $s_r$-th sampled time series.
\end{Dfn}
\vspace{-0.1in}

\begin{Dfn}
\textbf{Positive Query Set $\textbf{P}_i$}: we define $\textbf{P}_i = \{\textbf{p}_i^1,\cdots,\textbf{p}_i^{S_p}\} $ to denote the positive query set of user with size of $S_p$. Specifically, every entry $\textbf{p}_i^{s_p}$ represents the $s_p$-th sampled day-specific time series $\textbf{x}_i^t$ from user $u_i$.
\end{Dfn}

\vspace{-0.1in}
\begin{Dfn}
\textbf{Negative Query Set $\textbf{Q}_i$}: $\textbf{Q}_i$ is defined to as the negative query set for user $u_i$. Particularly, $\textbf{Q}_i = \{\textbf{q}_i^1,\cdots,\textbf{q}_i^{S_q}\}$ where $\textbf{q}_i^{s_q}$ is the sampled $s_q$-th day-specific time series from other users except user $u_{i'}$, \ie, $u_{i'} (i'\neq i)$.
\end{Dfn}
\vspace{-0.1in}

% In this subsection, we introduce the learning process of our developed \model\ framework. There have also been (semi-)supervised learning approaches for data classification in healthcare~\cite{che2017boosting,ma2018kame}. Basically these methods extract relevant features based on provided external labels (\eg, user health records) and learn a classifier to categorize the healthcare term pairs into relations or non-relations (\eg, risk relationships between users and diseases). However, in healthcare scenarios, the training data for (semi-)supervised methods are limited and insufficient to extract user-label relations~\cite{choi2017gram}. In contrast, we focus on the representation learning process in an unsupervised training setting when facing data insufficiency, to fit a more practical health-sensory data scenario.

% Our goal is to embed unlabeled health-sensory time series into low-dimensional spaces, in which every time series is represented as a low-dimensional vector. To address the training label scarcity problem, we design our model optimization framework with the exploration of intra-series temporal consistency. In particular, within a series of sensing data points (\eg, heart rate records), even though the measurements change over time, they do not change drastically within a short time period, since they belong to the same user~\cite{ukil2016heart}. For example, the heart rate measurements sampled from consecutive time intervals (\eg, day-long chunks) of the same people may a more similar distribution as compared to sampling from different people~\cite{bhattacharjee2018heart} \red{broken sentence}. Hence, in this work, we design a Siamese-triplet network optimization framework to capture such temporal consistency.

% The key idea of our Siamese-triplet network optimization framework is to learn representations with the constrain--making intra-series data point pairs closer to each other and inter-series data point pairs further apart. We first define the following terms to be used in our optimization framework.
% \begin{Dfn}
% \textbf{reference Set $S$}: we define $S_i$ to represent the sampled reference set of user $u_i$. In particular, $S_i = \{s_i^1,...,s_i^j,...,s_i^J\})$ (indexed by $j$), where $J$ is size of reference set corresponding to $J$ sampled days. In $S_i$, each element $s_i^j$ represents the health measurements of user $u_i$ from $j$-th sampled day-long chunks.
% \end{Dfn}

% \begin{Dfn}
% \textbf{Positive Query Set $P$}: we define $P_i$ to denote the positive query set of user $u_i$, \ie, $P_i = \{p_i^1,...,p_i^k,...,p_i^K\})$ with size of $K$. Specifically, every entry $p_i^k$ represents the user $u_i$'s health measurements from $k$-th sampled day-long chunks.
% \end{Dfn}

% \begin{Dfn}
% \textbf{Negative Query Set $Q$}: $Q_i$ is defined to represent the negative query set of user $u_i$. Particularly, $Q_i = \{q_i^1,...,q_i^r,...,q_i^r\})$ where $q_i^r$ is the sampled $\textbf{R}$-th day-long chunks from other users except user $u_i$, \ie, $u_{i'} (i'\neq i)$.
% \end{Dfn}

Based on the above definitions, given a specific user $u_i$, we estimate the similarity between his/her reference set $\textbf{r}_i$ and each query from his/her positive query set $\textbf{P}_i$ and negative query set $\textbf{Q}_i$. In particular, we first aggregate the elements from user $u_i$'s reference set $\textbf{S}_i$ as: $\widetilde{\mathbf{r}}_i=\textbf{A}(\textbf{R}_i)$, where $\textbf{A}(\cdot)$ is the aggregation function which represents the developed temporal pattern aggregation network. Then, we compute the cosine similarity of aggregated reference element $\widetilde{\mathbf{r}}_i$ and each query (\ie, $\textbf{p}_i^{s_p}$ and $\textbf{q}_i^{s_q}$) from the generated positive query set $\textbf{P}_i$ and negative query set $\textbf{Q}_i$. Formally, the similarity estimation function $\mathcal{S}$ is presented as follows:
\begin{align}
\mathcal{S}(\widetilde{\mathbf{r}}_i, \mathbf{p}_i^{s_p}) = \widetilde{\mathbf{r}}_i\cdot (E(\textbf{p}_i^{s_p}))^T; ~~s_p\in [1,...,S_p]; \nonumber\\
\mathcal{S}(\widetilde{\mathbf{r}}_i, \mathbf{q}_i^{s_q}) = \widetilde{\mathbf{r}}_i\cdot (E(\textbf{q}_i^{s_q}))^T; ~~s_q\in [1,...,S_q];
\end{align}
\noindent where $\mathcal{S}(\widetilde{\mathbf{r}}_i, \mathbf{p}_i^{s_p}) \in \mathbb{R}$ and $\mathcal{S}(\widetilde{\mathbf{r}}_i, \mathbf{q}_i^{s_q}) \in \mathbb{R}$. To capture the temporal consistency of each individual user $u_i$ and inconsistency among different users, we aim to learn latent representations which preserve inherent relationships between each user's reference set and query set, \ie, time series embeddings from the same user are closer to each other, while embeddings from different users are more differentiated from each other. More specifically, the similarity between the aggregated reference element $\widetilde{\mathbf{r}}_i$ and the positive query $\textbf{p}_i^{s_p}$ should be larger, while the similarity between $\widetilde{\mathbf{r}}_i$ and the negative query $\textbf{q}_i^{s_q}$ should be smaller, \ie, $\mathcal{S}(\widetilde{\mathbf{r}}_i,\textbf{p}_i^{s_p}) > \mathcal{S}(\widetilde{\mathbf{R}}_i, \textbf{q}_i^{s_q})$. Therefore, we formally define our loss function as follows:
\begin{align}
\mathcal{L}_{s}=  max(0, \mathcal{S}(\widetilde{\mathbf{r}}_i, \textbf{q}_i^{s_q})-\mathcal{S}(\widetilde{\mathbf{r}}_i, \textbf{p}_i^{s_p})+z)
\end{align}
\noindent where $z$ is the margin between two similarities. The objective function of joint model is defined as:
$\mathcal{L}_{joint} = \mathcal{L}_{ae} + \lambda \mathcal{L}_{s}$, where $\lambda$ is the coefficient which control the weight of Siamese-triplet loss. The model parameters can be derived by minimizing the loss function. We use Adam optimizer to learn the parameters of \model. The model optimization process is summarized in Algorithm~\ref{alg:model}. 

\begin{algorithm}
\small
% Define parameter notations
    \SetKwData{User}{$\mathbf{U}$}
    \SetKwData{Item}{$\mathbf{I}$}
    \SetKwData{OneUser}{u}
    \SetKwData{OneItem}{i}
    
    \SetKwData{Train}{$\mathbf{X}$}
    \SetKwData{TrainBatch}{$\mathsf{T_{batch}}$}
    \SetKwData{TrainBatch}{\textsf{QueryBatch}}
    
    \SetKwData{Rtrue}{${r}_{t,a_k}$}
    \SetKwData{Rpred}{$\hat{r}_{t,a_k}$}
    
    \SetKwData{Step}{$s$}
    \SetKwData{Batch}{$b_{\textsf{size}}$}
    \SetKwData{Support}{$S_{\textsf{size}}$}
    \SetKwData{Positive}{$P_{\textsf{size}}$}
    \SetKwData{Negative}{$N_{\textsf{size}}$}
    \SetKwData{classPerEpisode}{$N_c$}
    \SetKwFunction{Sample}{sample}
    
    \SetKwFunction{LSTM}{LSTM}
    \SetKwFunction{RandomWalk}{RandomWalk}
    \SetKwData{Null}{\textsf{NULL}}
    \SetKwData{LSTMRes}{c}
    \SetKwFunction{MLP}{MLP}
    \SetKwData{OtherPara}{$\theta$}
    \SetKwFunction{Projection}{Projection}
    
    \SetKwData{Loss}{$\mathcal{L}$}
    
    \SetKwInOut{Parameter}{Paras}

% Actual algorithm is here    
    \KwIn{User set $U$, batch size \Batch, support set size $S_r$, positive query size $S_p$, negative query size $S_q$}
    \emph{Initialize all parameters}\;
    % \tcp{Sample a minibatch of size \Batch.}
    \ForEach{batch}
    {
        sample a set of $\Batch$ users $V$ from User set $U$\; 
        \ForEach{user $u_i$ in $V$}
        {
            sample support set $\textbf{R}_i$ and positive set $\textbf{P}_i$ from $\textbf{X}_i$\;
            sample negative set $\textbf{Q}_i$ from $\textbf{X}_j$\;
            feed each entry in $\textbf{R}_i$, $\textbf{P}_i$ and $\textbf{Q}_i$ into autoencoder to get daily representations and compute $\mathcal{L}_{ae}$\; 
            aggregate support set $\textbf{R}_i$ and derive $\mathcal{L}_{s}$\; 
        }
        \emph{update all parameters w.r.t $\mathcal{L}_{joint}= \mathcal{L}_{ae} + \lambda \mathcal{L}_{s}$}\;
        % update loss~\Loss w.r.t $-\frac{1}{\Batch}\sum max(0, margin+\textsf{sim}_{r,n} -\textsf{sim}_{r,p})$\;
        % \emph{update all parameters w.r.t \Loss}\;
    }
    \caption{The Model Inference Process of \model.}
    \label{alg:model}
\end{algorithm}

\noindent \textbf{Unsupervised and semi-supervised learning scenarios}. Our \model\ is a general representation learning framework that is flexible for both unsupervised (without labeled training instances) and semi-supervised (limited number of labeled instances) learning. In semi-supervised learning, given the labeled time series and its target value, we take the learned representation vector as the input of a single-layer perceptrons with a combined loss function, \ie integrate the joint objective function $\mathcal{L}_{joint}$ with the loss function based on cross-entropy (categorical values) or MSE (quantitative values).

% Given a labeled time series x and its target value y, we can take the compressed temporal input vector as the input of a single layer perceptrons and add the correponding loss function(e.g., cross-entropy, MSE) to the total loss

% Based on the above definitions, given a specific time series $u_i$, we estimate the similarity between the reference set $S_i$ and each query from his/her positive query set $P_i$ and negative query set $S_i$. In particular, we first aggregate the elements from user $u_i$'s reference set $S_i$ as: $\widetilde{s}_i=\text{A}(S_i)$, where $A(\cdot)$ is the aggregation function. Then, we compute the cosine similarity~\cite{bayardo2007scaling} of aggregated reference element $\widetilde{s}_i$ and each query (\ie, $p_i^k$ and $q_i^r$) from the generated positive query set $P_i$ and negative query set $Q_i$ of user $u_i$. Formally, the similarity estimation function $\mathcal{S}$ is presented as follows:
% \begin{align}
% \mathcal{S}(\widetilde{s}_i, p_i^k) = \textbf{A}(f(S_i))\cdot f(p_i^k); ~~k\in [1,...,K] \nonumber\\
% \mathcal{S}(\widetilde{s}_i, q_i^r) = \textbf{A}(f(S_i))\cdot f(q_i^r); ~~r\in [1,...,R]
% \end{align}
% \noindent where $\cdot$ represents the dot product operation. In order to capture the temporal consistency of each individual user $u_i$, we aim to learn latent representations which preserve inherent relationships between each user's reference set and query set, \ie, health-sensing sampled day-long chunks from the same user are closer to each other, and sampled day-long chunks from different users are more separated from each other. More specifically, the similarity between the aggregated reference element $\widetilde{s}_i$ and the positive query $p_i^k$ should be larger, while the similarity between $\widetilde{s}_i$ and the negative query $q_i^r$ should be smaller, \ie, $\mathcal{S}(\widetilde{s}_i, p_i^k) > \mathcal{S}(\widetilde{s}_i, q_i^r)$. Therefore, we formally define our loss function as follows:
% \begin{align}
% \mathcal{L}_{s}=\frac{1}{I}\sum max(0, \mathcal{S}(\widetilde{s}_i, q_i^r)-\mathcal{S}(\widetilde{s}_i, p_i^k) +m)
% \end{align}
% \noindent where $m$ is the margin between two similarities. The model parameters can be derived by minimizing the loss function. In this work, we use Adam optimizer~\cite{le2011optimization} to learn the parameters of \model. The model optimization process is summarized in Algorithm~\ref{alg:model}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Backup-1%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Motif Extraction--time series Pre-processing} 

% The representation for heart rate data is still challenge with the fact that most people share very similar trends in each day. Supervision approach in deep learning technique provides a intuitive and effective way to learn effective representations by retaining the most relevant information to infer correct labels with back-propagation. However, as pointed in the introduction section, it is expensive to collect heart rate data with labeled health condition. 
% % To obtain the good embedding of heart rate time series data with arbitrary length, 
% Inspired by \cite{wang2015unsupervised}, we design a Siamese Triple Network based approach with ranking loss for unsupervised learning to train above encoder structure. Our key idea is the daily time series from same person provides supervision. Specifically, we distill heart rate representations such that the daily query heart rate data is closer to the reference/tracked heart rate data as compared to the other randomly sampled daily heart rate data (collected from other people).     

% We first give the following definitions used in the training process:
% %refer to the definition given in section 2.1 https://openreview.net/pdf?id=HJcSzz-CZ
% \begin{Dfn}
% \textbf{reference Set $\textbf{referenceSet}$} a reference set $S = {x_1, ..., x_{S_{size}}}$ containing $S_{size}$ examples sampled from the daily heart rate time series of person $u$.
% \end{Dfn}
% \begin{Dfn}
% \textbf{Positive Query Set $\textbf{PositiveSet}$} a Positive Query set $S = {x*_1, ..., x*_{Q_{size}}}$ containing $Q_{size}$ examples sampled from the daily heart rate time series from the same person $u$ in $\textbf{referenceSet}$.
% \end{Dfn}
% \begin{Dfn}
% \textbf{Negative Query Set $\textbf{NegativeSet}$} a Negative Query set $S = {x'_1, ..., x'_{N_{size}}}$ containing $N_{size}$ examples sampled from the daily heart rate time series from the rest people in the training dataset.
% \end{Dfn}
% Then, we define the similarity of reference set and each query based on the cosine similarity, which is commonly used in CV\cite{wang2015unsupervised} and NLP area: 
% \begin{align}
% \textbf{Sim}(\textbf{referenceSet}, q) = A(f(\textbf{referenceSet}))\cdot f(q)
% \end{align}
% \noindent where $A(\cdot)$ and $f(\cdot)$ respectively represents the function of aggregation and time series encoder, $\cdot$ is the dot product operation.The regularity of people's heart rate is prevalence, so we want the learned time series embedding is so that the similarity between reference set and the positive query is large and the similarity between reference set and other negative query is encouraged to be smaller. In another words, we want to enforce $\textbf{Sim}(\textbf{referenceSet}, x*)>\textbf{Sim}(\textbf{referenceSet}, x')$. Therefore, the loss of our ranking model is defined by hinge loss as:
% \begin{align}
% -\frac{1}{N}\sum max(0, m+\textbf{Sim}(\textbf{referenceSet}, x') -\textbf{Sim}(\textbf{referenceSet}, x*))
% \end{align}
% \noindent where m is the margin between two similarities.

% \subsection{Unstructured Embedding}
% The length of extracted time-series motifs typically varies form hundreds to thousands. Unequal and long lengths of motifs makes it difficult to learn representations which encodes different temporal pattern. Existing neural network-based time series pattern encoding models are not able to interpret the long-range dependencies in time series data due to computational efficiency, \ie, time-consuming gradient derivation as it is propagated back through time steps. To solve this issue, we propose first convert time-series motifs to image and then learn the low-dimensional representations of images with the neural network structure.  

% \subsubsection{Recurrent Plot+Edge Enhancement} 


% %Here is a survey paper which gives an overview about the state-of-the-art techniques on time series data preprocessing. (https://www.ncbi.nlm.nih.gov/pubmed/17111118)
% How to convert a single vector to the input of CNN model for analysis tasks on time series data?
% Recurrent Plot: The idea is as follows: let us denote the time series data by $(x_0, ..., x_n, ..., x_N)$, the return map will be a distance matrix $D\in R^{N\times N}$, which each element $D_{i,j}$  is derived by $dist(x_i,x_j)$. 


% \red{In this topic, the focus shifts to image analysis, which in some respects is a more difficult problem. Image analysis algorithms draw on information present within an image, or group of images, to extract properties about the scene being imaged. For example, in machine vision applications, images are analyzed to oftentimes determine the orientation of objects within the scene in order to send feedback to a robotic system. In medical imaging registration systems, radiographs, or slices from 3D volumes, are analyzed or fused together by a computerized system to glean information that a clinician or medical device may be interested in, such as the presence of tumors or the location and orientation of anatomical landmarks. In military tracking systems, interest lies in identifying targets, such landmarks, enemy combatants, etc. There are many other real-world applications where image analysis plays a large role.}



% \subsubsection{Convolutional Autoencoder} 
% % refer https://xifengguo.github.io/papers/ICONIP17-DCEC.pdf


% An autoencoder consists of two components, corresponding to encoder $f_W (\cdot)$ and decoder $g_U (\cdot)$ respectively. The encoder projects input data from a high dimensional input into the lower dimensional bottleneck layer, then the decoder takes the compressed input and converted back to the original input shape. It aims to find a compressed representation for each input sample by minimizing the mean squared errors (MSE) between its input and output over all samples as follows:
% \begin{align}
% \mathscr{L} =&  \sum_i  ||g_U (f_W (x_i))-\hat{x}_i||_2^2\nonumber\\
% f_W (x_i) =& \sigma(\cdots\sigma(\sigma(x_i*W_0)*W_1) \cdots*W_L)\nonumber\\
% g_U (h_i) =& \sigma(\cdots\sigma(\sigma(h_i*U_0)*U_1) \cdots*U_L) 
% \label{eq:loss_fun1}
% \end{align}
% \noindent where $i$ is the index of input samples, $*$ and $\sigma$ represent the activation function (e.g., $ReLU$ or $Tanh$ function) of convolutional layers and the convolutional operation, respectively. 

% \subsection{Structured Embedding}



% \subsection{Embedding Fusion}


% In particular, at the first step, we perform the convolution operation on the learned intermediate feature map representations from the previous layer. At the second step, a channel-wise recalibration gating mechanism is developed to automatically select the most informative elements from the encoded embedding vectors across different channels. We define $\alpha_{i,l} \in \mathbb{R}^{d_{\alpha}}$ to indicate the learned importance weight vector, where $d_c$ is the dimension size of $\alpha_{i,l}$ of the $l$-th block in this architecture. In $\alpha_{i,l}$, each element corresponds to the quantitative importance degree for each individual channel of the feature map representation. Then, we recalibrate the feature representation with the vector $\alpha_{i,l}$ by performing element-wise multiplication with feature representation $z^{i,l}$, to generate the recalibrated representation $\widetilde{z}_{i,l}$. Formally, the channel-wise gating mechanisam is represented as follows:
% \begin{align}
% \widetilde{z}_{i,l} = \sigma (\textbf{W}_2 \cdot \delta(\textbf{W}_1 \cdot \varphi))
% \end{align}
% In addition, in order to capture the inter-dependencies among temporal dimension, we further develop another temporal recalibration gating mechanism. More specifically, we define a temporal importance vector $\beta_{i,l}$ to interpret the importance of past time series data. We formally represent our proposed temporal gating mechanism as follows:
% \begin{align}
% \widetilde{v}_{i,l} = \sigma (\textbf{W}_2 \cdot \delta(\textbf{W}_1 \cdot \varphi))
% \end{align}

% We adopt auto-encoder pipeline for dimension reduction of time series. The encoder takes an daily-long time series and produces a latent feature representation of that image. The decoder takes this feature representation and reconstruct the input time series. To alleviate the influence of the missing segment of time series to representation learning, we propose XXX layer as the basic block in temporal Auto-encoder as shown in XXXX. For the l-th layer, initial feature map $V_l$ is the output of $(l âˆ’ 1)^{th}$ conv-layer. We first use the channel-wise attention gating mechanism to obtain the channel-wise attention weights $\alpha^l$, which are multiplied in channel-wise of the feature map. Then, we use the spatial attention function Î¦s to obtain the spatial attention weights $\beta^l$, which are multiplied in each temporal regions, resulting in an attentive feature map $Xl$. Finally, subsampling/max-pooling or upsampling operation is applied. 

%In particular, the channel and temporal gating mechanism is defined as follows: 

% \subsubsection{Channel-Wise Gating Mechanism}
% In our \model\ framework, to effectively interpret the feature representations, we propose to design a channel-wise gating mechanism to learn the importance of each individual channel.

% \subsubsection{Temporal Gating Mechanism}


% refer this squeeze and excitement
% application in http://openaccess.thecvf.com/content_cvpr_2017/papers/Chen_SCA-CNN_Spatial_and_CVPR_2017_paper.pdf
